ESOD: Efficient Small Object Detection on High-Resolution Images

Enlarging input images is a straightforward and effective approach to promote small object detection. However, simple image enlargement is significantly expensive on both computations and GPU memory. In fact, small objects are usually sparsely distributed and locally clustered. Therefore, massive feature extraction computations are wasted on the non-target background area of images. Recent works have tried to pick out target-containing regions using an extra network and perform conventional object detection, but the newly introduced computation limits their final performance. In this paper, we propose to reuse the detector's backbone to conduct feature-level object-seeking and patch-slicing, which can avoid redundant feature extraction and reduce the computation cost. Incorporating a sparse detection head, we are able to detect small objects on high-resolution inputs (e.g., 1080P or larger) for superior performance. The resulting Efficient Small Object Detection (ESOD) approach is a generic framework, which can be applied to both CNN- and ViT-based detectors to save the computation and GPU memory costs. Extensive experiments demonstrate the efficacy and efficiency of our method. In particular, our method consistently surpasses the SOTA detectors by a large margin (e.g., 8% gains on AP) on the representative VisDrone, UAVDT, and TinyPerson datasets. Code is available at https://github.com/alibaba/esod.

==> content/6_biography.tex <==

% \bf{If you will not include a photo:}\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/bio/kai_liu.jpg}}]
{Kai Liu}
received the B.S. degree from Zhejiang University, Hangzhou, China, in 2020, where he is currently pursuing the Ph.D. degree with the College of Biomedical Engineering and Instrument Science.
His research interests include computer vision and cross-modality learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/bio/zhihang_fu.jpg}}]
{Zhihang Fu}
received the B.S. and Ph.D. degrees from Zhejiang University, Hangzhou, China, in 2013 and 2019, respectively. He currently works in the Alibaba Cloud, Hangzhou. His research interests include deep learning and computer vision.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/bio/sheng_jin.jpg}}]
{Sheng Jin}
is currently a Research Fellow in S-Lab, Nanyang Technological University, Singapore. Before that, he received his B.S. degree in Applied Mathematic from Harbin Institute of Technology and the Ph.D. degree in Computer Science and Technology from Harbin Institute of Technology.  He also joined Alibaba Cloud as a Senior Algorithm Engineer. His research interests include computer vision and machine learning.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/bio/ze_chen.jpg}}]
{Ze Chen}
received the B.S. and Ph.D. degrees from Zhejiang University, Hangzhou, China, in 2016 and 2021, respectively. He currently works in the Alibaba Cloud, Hangzhou. His research interests include deep learning and computer vision.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/bio/fan_zhou.jpg}}]
{Fan Zhou}
received the B.Sc. and Ph.D. degrees from Zhejiang University, Hangzhou, China, in 2000 and 2006, respectively. He is currently a Professor of Zhejiang University. His major research fields are sonar signal processing and FPGA-based high-performance computing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/bio/rongxin_jiang.jpg}}]
{Rongxin Jiang}
received the B.S. and Ph.D. degrees in electrical engineering from the College of Biomedical Engineering \& Instrument Science, Zhejiang University, China, in 2002 and 2008, respectively, where He is currently an Associate Researcher. His research interests include embedded systems and computer vision.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/bio/yaowu_chen.jpg}}]
{Yaowu Chen}
received the Ph.D. degree rom Zhejiang University, Hangzhou, China, in 1998. He is currently a professor and the director of the Institute of Advanced Digital Technologies and Instrumentation, Zhejiang University. His major research fields are embedded systems, networking multimedia systems, and electronic instrumentation systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figure/bio/jieping_ye.png}}]
{Jieping Ye}
(Fellow, IEEE) is a VP of Alibaba Cloud and the Head of the Apsara Laboratory. His research interests include big data, machine learning, and artificial intelligence with applications in transportation, smart city, and biomedicine. He has served as a Senior Program Committee/Area Chair/Program Committee Vice Chair of many conferences including NeurlPS, ICML, KDD, IJCAI, ICDM, and SDM. He has served as an Associate Editor of Data Mining and Knowledge Discovery, IEEE Transactions on Knowledge and Data Engineering, and IEEE Transactions on Pattern Analysis and Machine Intelligence. He won the NSF CAREER Award in 2010. His papers have been selected for the outstanding student paper at ICML in 2004, the KDD best research paper runner-up in 2013, and the KDD best student paper award in 2014. He has also won first place in the 2019 INFORMS Daniel H. Wagner Prize, one of the top awards in operation research practice. Dr. Ye was elevated to an IEEE Fellow in 2019 and named an ACM Distinguished Scientist in 2020 for his contributions to the methodology and application of machine learning and data mining.
\end{IEEEbiography}

